Visco-potential free-surface flows and long wave modelling

In a recent study [DutykhDias2007] we presented a novel visco-potential free surface flows formulation. The governing equations contain local and nonlocal dissipative terms. From physical point of view, local dissipation terms come from molecular viscosity but in practical computations, rather eddy viscosity should be used. On the other hand, nonlocal dissipative term represents a correction due to the presence of a bottom boundary layer. Using the standard procedure of Boussinesq equations derivation, we come to nonlocal long wave equations. In this article we analyse dispersion relation properties of proposed models. The effect of nonlocal term on solitary and linear progressive waves attenuation is investigated. Finally, we present some computations with viscous Boussinesq equations solved by a Fourier type spectral method.

==> Figs/Nonlocal/regions.tex <==
%%Created by jPicEdt 1.4.1: mixed JPIC-XML/LaTeX format
%%Sat May 19 08:25:23 CEST 2007
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.87" x-max="65.62" y-min="-3.75" y-max="23.12" auto-bounding="true">
%<g>
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 points= "(28.75,23.12);(28.75,23.12);(28.75,9.38);(28.75,9.38)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(25.62,22.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$z$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(1.87,15.62);(1.87,15.62);(65.62,15.62);(65.62,15.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(63.12,13.12)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$x$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25.63,13.12)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$O$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(9.37,20.62)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$S_f$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.87,7.5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$R_i$
%</text>
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(41.25,0);(41.25,0);(41.25,-3.12);(41.25,-3.12)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(41.25,1.88);(41.25,1.88);(41.25,6.25);(41.25,6.25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,5)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$R_b$
%</text>
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(49.37,15.62);(49.37,15.62);(49.37,19.38);(49.37,19.38)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(49.37,13.75);(49.37,13.75);(49.37,10);(49.37,10)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(51.87,11.25)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$R_f$
%</text>
%<multicurve right-arrow= "head"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(14.37,14.38);(14.37,14.38);(14.37,1.88);(14.37,1.88)"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 smoothness= "0.7;0.7;0.7;0.7;0.7;0.7;0.7;0.7;0.7;0.7;0.7;0.7;0.7"
%	 points= "(1.87,15.62);(8.13,18.75);(11.87,17.5);(15.63,15.62);(23.75,16.25);(29.37,18.12);
%	(37.5,19.38);(43.13,16.88);(50.63,15);(55.63,18.12);(60.63,18.75);(61.87,18.12);
%	(61.87,18.12)"
%	 />
%<smoothpolygon stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 closed= "false"
%	 stroke-width= "0.2"
%	 smoothness= "0.7;0.7;0.7;0.7;0.7;0.7;0.7;0.7;0.7;0.7;0.7;0.7;0.7"
%	 stroke-style= "dashed"
%	 points= "(1.87,13.75);(8.12,16.88);(11.87,15.62);(15.62,13.75);(23.75,14.38);(29.37,16.25);
%	(37.5,17.5);(43.12,15);(50.62,13.12);(55.62,16.25);(60.62,16.88);(61.87,16.25);
%	(61.87,16.25)"
%	 />
%<smoothpolygon stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 closed= "false"
%	 stroke-width= "0.2"
%	 smoothness= "0.7;0.7;0.7;0.7;0.7;0.7"
%	 stroke-style= "dashed"
%	 points= "(1.87,-1.88);(11.87,3.12);(26.87,-1.88);(41.87,3.12);(61.87,-1.88);(61.87,-1.88)"
%	 />
%<smoothpolygon fill-style= "none"
%	 closed= "false"
%	 stroke-width= "0.35"
%	 smoothness= "0.7;0.7;0.7;0.7;0.7;0.7"
%	 points= "(1.87,-3.75);(11.87,1.25);(26.87,-3.75);(41.87,1.25);(61.87,-3.75);(61.87,-3.75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(12.5,-3.75)"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 >
%$S_b$
%</text>
%</g>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(65.62,23.12)(0,0)
\linethickness{0.3mm}
\put(28.75,9.38){\line(0,1){13.74}}
\put(28.75,23.12){\vector(0,1){0.12}}
\put(25.62,22.5){\makebox(0,0)[cc]{$z$}}

\linethickness{0.3mm}
\put(1.87,15.62){\line(1,0){63.75}}
\put(65.62,15.62){\vector(1,0){0.12}}
\put(63.12,13.12){\makebox(0,0)[cc]{$x$}}

\put(25.63,13.12){\makebox(0,0)[cc]{$O$}}

\put(9.37,20.62){\makebox(0,0)[cc]{$S_f$}}

\put(16.87,7.5){\makebox(0,0)[cc]{$R_i$}}

\linethickness{0.15mm}
\put(41.25,-3.12){\line(0,1){3.12}}
\put(41.25,0){\vector(0,1){0.12}}
\linethickness{0.15mm}
\put(41.25,1.88){\line(0,1){4.37}}
\put(41.25,1.88){\vector(0,-1){0.12}}
\put(45,5){\makebox(0,0)[cc]{$R_b$}}

\linethickness{0.15mm}
\put(49.37,15.62){\line(0,1){3.76}}
\put(49.37,15.62){\vector(0,-1){0.12}}
\linethickness{0.15mm}
\put(49.37,10){\line(0,1){3.75}}
\put(49.37,13.75){\vector(0,1){0.12}}
\put(51.87,11.25){\makebox(0,0)[cc]{$R_f$}}

\linethickness{0.15mm}
\put(14.37,1.88){\line(0,1){12.5}}
\put(14.37,14.38){\vector(0,1){0.12}}
\put(14.37,1.88){\vector(0,-1){0.12}}
\linethickness{0.3mm}
\qbezier(1.87,15.62)(5.13,17.26)(7.09,17.86)
\qbezier(7.09,17.86)(9.04,18.46)(10,18.12)
\qbezier(10,18.12)(10.97,17.8)(11.87,17.43)
\qbezier(11.87,17.43)(12.77,17.05)(13.75,16.56)
\qbezier(13.75,16.56)(14.72,16.07)(16.15,15.92)
\qbezier(16.15,15.92)(17.58,15.77)(19.69,15.94)
\qbezier(19.69,15.94)(21.8,16.1)(23.45,16.4)
\qbezier(23.45,16.4)(25.11,16.7)(26.56,17.19)
\qbezier(26.56,17.19)(28.01,17.67)(29.67,18.05)
\qbezier(29.67,18.05)(31.32,18.42)(33.44,18.75)
\qbezier(33.44,18.75)(35.55,19.08)(37.2,18.93)
\qbezier(37.2,18.93)(38.86,18.78)(40.32,18.13)
\qbezier(40.32,18.13)(41.77,17.48)(43.35,16.95)
\qbezier(43.35,16.95)(44.93,16.43)(46.88,15.94)
\qbezier(46.88,15.94)(48.83,15.44)(50.33,15.59)
\qbezier(50.33,15.59)(51.84,15.74)(53.13,16.56)
\qbezier(53.13,16.56)(54.43,17.37)(55.63,17.82)
\qbezier(55.63,17.82)(56.83,18.28)(58.13,18.44)
\qbezier(58.13,18.44)(59.43,18.6)(60.18,18.6)
\qbezier(60.18,18.6)(60.93,18.6)(61.25,18.44)
\qbezier(61.25,18.44)(61.57,18.27)(61.72,18.19)
\qbezier(61.72,18.19)(61.87,18.12)(61.87,18.12)
\linethickness{0.2mm}
\qbezier(1.87,13.75)(5.13,15.39)(7.08,15.99)
\qbezier(7.08,15.99)(9.04,16.59)(10,16.25)
\qbezier(10,16.25)(10.97,15.92)(11.87,15.55)
\qbezier(11.87,15.55)(12.77,15.17)(13.75,14.69)
\qbezier(13.75,14.69)(14.71,14.2)(16.14,14.05)
\qbezier(16.14,14.05)(17.57,13.9)(19.69,14.06)
\qbezier(19.69,14.06)(21.8,14.23)(23.45,14.53)
\qbezier(23.45,14.53)(25.11,14.83)(26.56,15.31)
\qbezier(26.56,15.31)(28.01,15.8)(29.67,16.18)
\qbezier(29.67,16.18)(31.32,16.55)(33.44,16.88)
\qbezier(33.44,16.88)(35.55,17.21)(37.2,17.05)
\qbezier(37.2,17.05)(38.86,16.9)(40.31,16.25)
\qbezier(40.31,16.25)(41.76,15.6)(43.34,15.07)
\qbezier(43.34,15.07)(44.92,14.55)(46.87,14.06)
\qbezier(46.87,14.06)(48.82,13.56)(50.32,13.71)
\qbezier(50.32,13.71)(51.83,13.87)(53.12,14.69)
\qbezier(53.12,14.69)(54.42,15.5)(55.62,15.95)
\qbezier(55.62,15.95)(56.82,16.41)(58.12,16.56)
\qbezier(58.12,16.56)(59.42,16.73)(60.17,16.73)
\qbezier(60.17,16.73)(60.93,16.73)(61.25,16.56)
\qbezier(61.25,16.56)(61.57,16.4)(61.72,16.32)
\qbezier(61.72,16.32)(61.87,16.25)(61.87,16.25)
\linethickness{0.2mm}
\qbezier(1.87,-1.88)(7.07,0.74)(11.28,1.34)
\qbezier(11.28,1.34)(15.49,1.94)(19.37,0.62)
\qbezier(19.37,0.62)(23.26,-0.69)(26.87,-0.69)
\qbezier(26.87,-0.69)(30.48,-0.69)(34.37,0.62)
\qbezier(34.37,0.62)(38.25,1.93)(42.46,1.93)
\qbezier(42.46,1.93)(46.67,1.93)(51.87,0.62)
\qbezier(51.87,0.62)(57.09,-0.68)(59.5,-1.29)
\qbezier(59.5,-1.29)(61.9,-1.89)(61.87,-1.88)
\linethickness{0.35mm}
\qbezier(1.87,-3.75)(7.07,-1.13)(11.28,-0.53)
\qbezier(11.28,-0.53)(15.49,0.07)(19.37,-1.25)
\qbezier(19.37,-1.25)(23.26,-2.56)(26.87,-2.56)
\qbezier(26.87,-2.56)(30.48,-2.56)(34.37,-1.25)
\qbezier(34.37,-1.25)(38.25,0.06)(42.46,0.06)
\qbezier(42.46,0.06)(46.67,0.06)(51.87,-1.25)
\qbezier(51.87,-1.25)(57.09,-2.55)(59.5,-3.16)
\qbezier(59.5,-3.16)(61.9,-3.76)(61.87,-3.75)
\put(12.5,-3.75){\makebox(0,0)[cc]{$S_b$}}

\end{picture}

